Contextual Equivalence for Signal Flow Graphs

We extend the signal flow calculus---a compositional account of the classical signal flow graph model of computation---to encompass affine behaviour, and furnish it with a novel operational semantics. The increased expressive power allows us to define a canonical notion of contextual equivalence, which we show to coincide with denotational equality. Finally, we characterise the realisable fragment of the calculus: those terms that express the computations of (affine) signal flow graphs.

==> TrajLaurent.tex <==
\section{From trajectories to Laurent series}

Trajectories are just Laurent series in disguise.
Each computation with runtime context defines a vector in $\laur^n \times \laur^m$, i.e., a pair of tuples of Laurent series in a straightforward way: for example, for a $(1,1)$ circuit $c$, the trajectory given by the infinite computation 
\[\context{p} c_0 \dtrans{u_0}{v_0} c_1 \dtrans{u_1}{v_1}  c_2 \dtrans{u_2}{v_2} c_3 \dtrans{u_3}{v_3} \dots\]
can be mapped to the pair of Laurent series $(\sigma,\tau)$ where $\sigma(i) = u_{i-p}$ and $\tau(i) = v_{i-p}$ for $i \geq m$ and $\sigma(i) = \tau(i) = 0$ otherwise.

More generally, given a $(n,m)$-trajectory $\sigma$, we can just reorganise the components of each step of the trajectory to obtain a pair of vectors $L(\sigma)\in\laur^n \times \laur^m$,
$$\left({\small\left( \begin{array}{c}
				  \!\alpha^1\! \\
				  \vdots\\
				  \!\alpha^n\!
				\end{array}\right)}, \,
{\small\left(%
				\begin{array}{c}
				  \!\beta^1\! \\
				  \vdots\\
				  \!\beta^m\!
				\end{array}\right)}\right)$$
where
%
\begin{equation}\label{eq:L-left}
\alpha^j(i)= \sigma_l(i)^j \qquad \beta^l(i) = \sigma_r(i)^l
\end{equation}
where $\sigma_l(i)^j$ (resp. $\sigma_r(i)^k$) denotes the $j$th (resp. $k$th) component of $\sigma_l(i)$ (resp. $\sigma_r(i)$), for $1\leq j\leq n$ (resp. $1\leq l\leq m$) and all $i\in\Z$.
Clearly, this operation is functorial and respects the monoidal product. 
\begin{theorem}\marginpar{RP: not sure whether we need to still prove it. It's obvious and tedious.}
$L\colon  \PTR \to \Rellaur$ is a morphism of props.
\end{theorem}

\begin{theorem}\label{thm:main}
$L \circ \osem{\cdot}=\dsem{\cdot}$
\end{theorem}
\begin{proof}
Since both are monoidal functors, it is enough to check the statement for the generators. 
\end{proof}
\begin{corollary}\label{cor:dsemexperiments}
Let $c\in \ACD[0,0]$. Then
$\dsem{c}=id_0$ iff $c\uparrow$.
\end{corollary}
\begin{proof}
By Proposition \ref{prop:twopossibility}, either $\dsem{c}=id_0$ or $\dsem{c}=\emptyset$, which by mean of Theorem \ref{thm:main} means that  $L\circ \osem{c}=id_0$ or $L \circ \osem{c}=\emptyset$. By definition of $L$ this means that either $\osem{c}$ contains a pointed trace or not. In the first case $c\uparrow$; in the second $ \not {c \uparrow}$.
\end{proof}
\section{From trajectories to Laurent series}

Trajectories are just Laurent series in disguise.
Each computation with runtime context defines a vector in $\laur^n \times \laur^m$, i.e., a pair of tuples of Laurent series in a straightforward way: for example, for a $(1,1)$ circuit $c$, the trajectory given by the infinite computation 
\[\context{p} c_0 \dtrans{u_0}{v_0} c_1 \dtrans{u_1}{v_1}  c_2 \dtrans{u_2}{v_2} c_3 \dtrans{u_3}{v_3} \dots\]
can be mapped to the pair of Laurent series $(\sigma,\tau)$ where $\sigma(i) = u_{i-p}$ and $\tau(i) = v_{i-p}$ for $i \geq m$ and $\sigma(i) = \tau(i) = 0$ otherwise.

More generally, given a $(n,m)$-trajectory $\sigma$, we can just reorganise the components of each step of the trajectory to obtain a pair of vectors $L(\sigma)\in\laur^n \times \laur^m$,
$$\left({\small\left( \begin{array}{c}
				  \!\alpha^1\! \\
				  \vdots\\
				  \!\alpha^n\!
				\end{array}\right)}, \,
{\small\left(%
				\begin{array}{c}
				  \!\beta^1\! \\
				  \vdots\\
				  \!\beta^m\!
				\end{array}\right)}\right)$$
where
%
\begin{equation}\label{eq:L-left}
\alpha^j(i)= \sigma_l(i)^j \qquad \beta^l(i) = \sigma_r(i)^l
\end{equation}
where $\sigma_l(i)^j$ (resp. $\sigma_r(i)^k$) denotes the $j$th (resp. $k$th) component of $\sigma_l(i)$ (resp. $\sigma_r(i)$), for $1\leq j\leq n$ (resp. $1\leq l\leq m$) and all $i\in\Z$.
Clearly, this operation is functorial and respects the monoidal product. 
\begin{theorem}\marginpar{RP: not sure whether we need to still prove it. It's obvious and tedious.}
$L\colon  \PTR \to \Rellaur$ is a morphism of props.
\end{theorem}

\begin{theorem}\label{thm:main}
$L \circ \osem{\cdot}=\dsem{\cdot}$
\end{theorem}
\begin{proof}
Since both are monoidal functors, it is enough to check the statement for the generators. 
\end{proof}
\begin{corollary}\label{cor:dsemexperiments}
Let $c\in \ACD[0,0]$. Then
$\dsem{c}=id_0$ iff $c\uparrow$.
\end{corollary}
\begin{proof}
By Proposition \ref{prop:twopossibility}, either $\dsem{c}=id_0$ or $\dsem{c}=\emptyset$, which by mean of Theorem \ref{thm:main} means that  $L\circ \osem{c}=id_0$ or $L \circ \osem{c}=\emptyset$. By definition of $L$ this means that either $\osem{c}$ contains a pointed trace or not. In the first case $c\uparrow$; in the second $ \not {c \uparrow}$.
\end{proof}

